Convolution identities for divisor sums and modular forms

We prove exact identities for convolution sums of divisor functions of the form $\sum_{n_1 \in \mathbb{Z} \smallsetminus \{0,n\}}\varphi(n_1,n-n_1)\sigma_{2m_1}(n_1)\sigma_{2m_2}(n-n_1)$ where $\varphi(n_1,n_2)$ is a Laurent polynomial with logarithms for which the sum is absolutely convergent. Such identities are motivated by computations in string theory and prove and generalize a conjecture of Chester, Green, Pufu, Wang, and Wen from \cite{CGPWW}. Originally, it was suspected that such sums, suitably extended to $n_1\in\{0,n\}$ should vanish, but in this paper we find that in general they give Fourier coefficients of holomorphic cusp forms.

==> makros.tex <==

\newcommand{\setmid}{\,:\,}


\DeclareMathOperator{\arcosh}{arcosh}
\DeclareMathOperator{\Hyp}{Hyp}
\DeclareMathOperator{\Conj}{Conj}
\DeclareMathOperator{\nte}{\mathbf{e}}

%BLZ
\DeclareMathOperator{\SFE}{SEF}
\DeclareMathOperator{\FFE}{FEF}






\newcommand{\TO}{\mc L}
\newcommand{\MTO}{\mc M}
\DeclareMathOperator{\s}{s}
\DeclareMathOperator{\sinc}{sinc}
\newcommand{\op}{\text{op}}



\newcommand{\llequiv}{[[}
\newcommand{\rrequiv}{]]}
\newcommand{\mapeins}{\phi_1}
\newcommand{\mapeinsn}{\phi_{1,n}}
\newcommand{\mapeinseins}{\phi_{1,1}}
\newcommand{\mapzwei}{\phi_2}
\newcommand{\mapzwein}{\phi_{2,n}}
\newcommand{\mgf}{\tau}
\newcommand{\mapdrei}{\psi_1}
\newcommand{\mapdrein}{\psi_{1,n}}
\newcommand{\mapvier}{\psi_2}
\newcommand{\mapviern}{\psi_{2,n}}

\DeclareMathOperator{\discr}{discr}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\bdinterval}{bdinterval}
\DeclareMathOperator{\interval}{interval}
\DeclareMathOperator{\level}{level}
\DeclareMathOperator{\Dis}{Dis}

\DeclareMathOperator{\UGeo}{UGeo}
\DeclareMathOperator{\PGeo}{PGeo}



\DeclareMathOperator{\FP}{FP}
\DeclareMathOperator{\POQF}{POQF}
\DeclareMathOperator{\OQF}{OQF}
\DeclareMathOperator{\Primlength}{PL}

\DeclareMathOperator{\base}{base}
\newcommand{\homsp}{\mathcal X}
\DeclareMathOperator{\Li}{Li}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\WF}{WF}
\newcommand{\bT}{\mathbf T}
\DeclareMathOperator{\Gen}{Gen}
\newcommand{\redu}{\text{red}}
% orbifolds

\DeclareMathOperator{\Eff}{Eff}
\DeclareMathOperator{\germ}{germ}
\DeclareMathOperator{\Germ}{Germ}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\Diff}{Diff}
\DeclareMathOperator{\Emb}{Emb}
\DeclareMathOperator{\Orbmap}{Orb}
\newcommand{\pullback}[2]{\,{}_{#1}\!\!\times_{#2}}
\DeclareMathOperator{\Agr}{Agr}

% algebraische Strukturen

\DeclareMathOperator{\Isom}{Isom}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Morph}{Morph}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Bil}{Bil}
\DeclareMathOperator{\QF}{QF}
\DeclareMathOperator{\Op}{Op}
\DeclareMathOperator{\Object}{Ob}
\DeclareMathOperator{\Spann}{Spann}
\DeclareMathOperator{\spann}{span}
\DeclareMathOperator{\ER}{ER}
\DeclareMathOperator{\Rang}{Rang}
\DeclareMathOperator{\Gal}{Gal}
\newcommand{\vs}{\text{vs}}
\newcommand{\Res}{\text{res}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Lie}{Lie}

%Standardmatrizen 

\DeclareMathOperator{\Mat}{Mat}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\AGL}{AGL}
\DeclareMathOperator{\Gl}{GL}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\PSL}{PSL}
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\PU}{PU}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Sp}{Sp}
\DeclareMathOperator{\PSp}{PSp}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\PSO}{PSO}
\DeclareMathOperator{\Orth}{O}
\DeclareMathOperator{\Spin}{Spin}
\DeclareMathOperator{\PGamma}{P\Gamma}

\DeclareMathOperator{\diag}{diag}

% Operatoren

\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\Rea}{Re}
\DeclareMathOperator{\sgn}{sgn}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\Bild}{Bild}

\DeclareMathOperator{\pr}{pr}
\DeclareMathOperator{\res}{res}
% besondere Matrizen

\DeclareMathOperator{\red}{Red}
\DeclareMathOperator{\I}{I}
%\newcommand{\I}{\mathds{1}}


% Lietheorie

\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\AD}{\textbf{Ad}}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\fsl}{\mathfrak{sl}}

% Wirkungen

\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\VS}{VS}

% Masse
\DeclareMathOperator{\HB}{HB}
\DeclareMathOperator{\cusp}{cusp}

% symbolische Dynamik

\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\Ext}{ext}
\DeclareMathOperator{\Int}{int}
\DeclareMathOperator{\height}{ht}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\Cod}{Cod}
\DeclareMathOperator{\NC}{NC}
\DeclareMathOperator{\D}{D}
\DeclareMathOperator{\MD}{MD}
\DeclareMathOperator{\Prim}{P}
\DeclareMathOperator{\Rel}{Rel}
\DeclareMathOperator{\HT}{HT}
\DeclareMathOperator{\vb}{vb}
\DeclareMathOperator{\vc}{vc}
\DeclareMathOperator{\bd}{bd}
\DeclareMathOperator{\BS}{BS}
\DeclareMathOperator{\CS}{CS}
\DeclareMathOperator{\DS}{DS}
\DeclareMathOperator{\IS}{IS}
\DeclareMathOperator{\NIC}{NIC}
\DeclareMathOperator{\Sides}{Sides}
\DeclareMathOperator{\Seq}{Seq}
\DeclareMathOperator{\cyl}{cyl}
\DeclareMathOperator{\IN}{IN}
\DeclareMathOperator{\sym}{sym}
\DeclareMathOperator{\Per}{Per}
\DeclareMathOperator{\ES}{ES}

\newcommand{\hg}{\overline \h^g}
\newcommand{\chg}{\cl_{\overline \h^g}}
\newcommand{\bhg}{\partial_g}

\newcommand{\dg}{\overline D^g}
\newcommand{\fcs}{\CS'\hspace{-.9mm}\big(\wt\fch_{\choices,\shmap}\big)}

\newcommand{\rueck}{\hspace{-.9mm}}

\newcommand{\fd}{\mc F}
\newcommand{\pch}{\mc A}
\newcommand{\fpch}{\mathbb A}
\newcommand{\ch}{\mc B}
\newcommand{\fch}{\mathbb B}
\newcommand{\choices}{\mathbb S}
\newcommand{\shmap}{\mathbb T}
\newcommand{\leer}{\Diamond}

\newcommand{\rd}{\text{red}}
\newcommand{\st}{\text{st}}
\newcommand{\all}{\text{all}}
\newcommand{\bk}{\text{bk}}
\newcommand{\tw}{\text{tw}}
\newcommand{\dec}{\text{dec}}
\newcommand{\parab}{\text{par}}
\newcommand{\dyn}{\text{dyn}}
% Buchstaben

\newcommand\F{\mathbb{F}}
\newcommand\N{\mathbb{N}}
\newcommand\Q{\mathbb{Q}}
\newcommand\R{\mathbb{R}}
\newcommand\Z{\mathbb{Z}}
\newcommand\C{\mathbb{C}}
\newcommand\dD{\mathbb{D}}
\newcommand{\h}{\mathbb{H}}
\newcommand{\mP}{\mathbb{P}}
\newcommand\T{\mathbb{T}}

\newcommand{\mc}[1]{\mathcal #1}
\newcommand{\mf}[1]{\mathfrak #1}
\newcommand{\mb}[1]{\mathbb #1}
\newcommand{\mft}[2]{\mathfrak #1\mathfrak #2}
\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}

\newcommand{\eps}{\varepsilon}
\newcommand\gG{\Gamma}
\newcommand\gd{\delta}



% speziell fuer SL2R
\DeclareMathOperator{\Pe}{P}
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\lsp}{lsp}
\DeclareMathOperator{\grp}{grp}
\DeclareMathOperator{\dvol}{dvol}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Orb}{\mc O}
\DeclareMathOperator{\mult}{mult}
\DeclareMathOperator{\Arcosh}{Arcosh}
\DeclareMathOperator{\arccot}{arccot}



% Koecher

\DeclareMathOperator{\RMod}{R-mod}
\DeclareMathOperator{\Ob}{Ob}

% FT
\DeclareMathOperator{\ind}{ind}

%BLZ
\DeclareMathOperator{\FE}{FE}

% Sonstiges

\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\M}{M}
\DeclareMathOperator{\Graph}{graph}
\DeclareMathOperator{\Fct}{Fct}
\DeclareMathOperator{\MCF}{MCF}
\DeclareMathOperator{\vN}{vN}

\DeclareMathOperator{\esssup}{ess\,sup}

% \newcommand{\sceq}{\mathrel{\mathop:}=}
% \newcommand{\seqc}{\mathrel{=\mkern-4.5mu{\mathop:}}}
\newcommand{\sceq}{\coloneqq}
\newcommand{\seqc}{\eqqcolon}

\newcommand{\mat}[4]{\begin{pmatrix} #1&#2\\#3&#4\end{pmatrix}}
\newcommand{\bmat}[4]{\begin{bmatrix} #1&#2\\#3&#4\end{bmatrix}}
\newcommand{\textmat}[4]{\left(\begin{smallmatrix} #1&#2 \\ #3&#4
\end{smallmatrix}\right)}
\newcommand{\textbmat}[4]{\left[\begin{smallmatrix} #1&#2 \\ #3&#4
\end{smallmatrix}\right]}
\newcommand{\vvek}[2]{\begin{pmatrix} #1 \\ #2 \end{pmatrix}}
\newcommand{\hvek}[2]{\begin{pmatrix} #1 & #2 \end{pmatrix}}

\newcommand\ie{\mbox{i.\,e., }}
\newcommand\eg{\mbox{e.\,g., }}
\newcommand\wrt{\mbox{w.\,r.\,t.\@ }}
\newcommand\Wlog{\mbox{w.\,l.\,o.\,g.\@ }}
\newcommand\resp{\mbox{resp.\@}}

\newcommand\abstand{\vspace{0.5cm}}
\newcommand\negab{\vspace{-0.5cm}}

\DeclareMathOperator{\ggt}{ggt}

\newcommand\mminus{\!\smallsetminus\!}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Commands from Ksenia
\newcommand\bs{\backslash}
\newcommand\norm{\textnormal{norm}}

\newcommand\HF{{}_{2}F_{1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
